Modeling Bitcoin Contracts by Timed Automata

Bitcoin is a peer-to-peer cryptographic currency system. Since its introduction in 2008, Bitcoin has gained noticeable popularity, mostly due to its following properties: (1) the transaction fees are very low, and (2) it is not controlled by any central authority, which in particular means that nobody can "print" the money to generate inflation. Moreover, the transaction syntax allows to create the so-called contracts, where a number of mutually-distrusting parties engage in a protocol to jointly perform some financial task, and the fairness of this process is guaranteed by the properties of Bitcoin. Although the Bitcoin contracts have several potential applications in the digital economy, so far they have not been widely used in real life. This is partly due to the fact that they are cumbersome to create and analyze, and hence risky to use. In this paper we propose to remedy this problem by using the methods originally developed for the computer-aided analysis for hardware and software systems, in particular those based on the timed automata. More concretely, we propose a framework for modeling the Bitcoin contracts using the timed automata in the UPPAAL model checker. Our method is general and can be used to model several contracts. As a proof-of-concept we use this framework to model some of the Bitcoin contracts from our recent previous work. We then automatically verify their security in UPPAAL, finding (and correcting) some subtle errors that were difficult to spot by the manual analysis. We hope that our work can draw the attention of the researchers working on formal modeling to the problem of the Bitcoin contract verification, and spark off more research on this topic.

==> BTC-commit.tex <==
% !TEX root = paper.tex

\newpage

\section{The \UPPAAL{} declarations in the model for the timed commitment scheme}\label{app:BTCcommit}

{\footnotesize
\begin{Verbatim}[numbers=left,numbersep=3pt]
// DECLARATIONS

const int KEYS_NUM = 2;
const int SECRETS_NUM = 1;
const int NSS_NUM = 1; //NON_STANDARD_SCRIPTS
const int PARTIES_NUM = 2 + 1; // + ADVERSARY
const int PROT_TX_NUM = 4;
const int NONCE_NUM = 2;
const int TX_NUM = 2 * PROT_TX_NUM;
const int KNOWN_SIGNATURES_SIZE = 1;
const int C_KEY = 0;
const int R_KEY = 1;
const int C_SEC = 0;
const int MAX_LATENCY = 10;
const int TIMERS_NUM = 1;
const int PROT_TIMELOCK = 100;
clock time;
int timer_t[TIMERS_NUM] = {PROT_TIMELOCK - MAX_LATENCY};
bool timer_passed[TIMERS_NUM];

typedef int[0,KEYS_NUM-1] Key;
typedef int[0,SECRETS_NUM-1] Secret;
typedef int[0,NSS_NUM-1] Nss;
typedef int[0,PARTIES_NUM-1] PartyId;
typedef int[0,TX_NUM-1] TxId;
typedef int[0,NONCE_NUM-1] Nonce;
typedef int[0,TIMERS_NUM-1] Timer;
typedef int[0,4] Status;

const PartyId ALICE = 0;
const PartyId BOB = 1;
const PartyId ADVERSARY = PARTIES_NUM - 1;

const Status UNSENT = 0;
const Status SENT = 1;
const Status CONFIRMED = 2;
const Status SPENT = 3;
const Status CANCELED = 4;

typedef struct {
  Key key;
  TxId tx_num;
  Nonce input_nonce;
} Signature;

typedef struct {
    bool standard;
    Key key;
    Nss script;
} OutputScript;

typedef struct {
  TxId num;
  TxId input;
  Status status;
  OutputScript out_script;
  int value;
  int timelock;
  bool timelock_passed;
  Nonce nonce;
  bool reveals_secret;
  Secret secret_revealed;
} Tx;

Tx bc[TX_NUM];
clock bc_clock[TX_NUM];
urgent chan urg_chan, signature;

typedef struct {
  bool know_key[KEYS_NUM];
  bool know_secret[SECRETS_NUM];
  int[0,KNOWN_SIGNATURES_SIZE] known_signatures_size;
  Signature known_signatures[KNOWN_SIGNATURES_SIZE];
} Party;

Party parties[PARTIES_NUM];

Signature create_signature(Key key, TxId tx_num, Nonce input_nonce) {
  Signature res = {key, tx_num, input_nonce};
  return res;
}

Signature create_signature_tx(Key key, Tx t) {
    return create_signature(key, t.num, bc[t.input].nonce);
}

void add_signature(Party& p, Signature s) {
  p.known_signatures[p.known_signatures_size++] = s;
}

void broadcast_signature(Signature s) {
  for(i : PartyId)
    add_signature(parties[i], s);
}

OutputScript create_standard_output_script(Key key) {
  OutputScript res = {true, key, 0};
  return res;
}

OutputScript create_nss(Nss nss) {
  OutputScript res = {false, 0, nss};
  return res;
}

Tx create_standard_tx(TxId num, TxId input, Key recipient) {
  Tx res;
  Tx in = bc[input];
  res.num = num;
  res.input = input;
  res.value = in.value;
  res.out_script = create_standard_output_script(recipient);
  return res;
}

bool was_malled(Tx t) {
  return t.nonce != 0;
}

bool is_waiting(Tx t) {
  return t.status == SENT;
}

bool is_valid(Tx t) {
  return t.timelock_passed and bc[t.input].status == CONFIRMED;
}

void confirm(Tx& t, Nonce n) {
  t.status = CONFIRMED;
  t.nonce = n;
  bc[t.input].status = SPENT;
}

void cancel(Tx& t) {
  t.status = CANCELED;
}

void try_to_confirm(Tx& t, Nonce n) {
  if(is_valid(t))
    confirm(t, n);
  else
    cancel(t);
}

void send(Tx& t) {
  t.status = SENT;
  bc_clock[t.num] = 0;
  if(t.reveals_secret)
    for(i : PartyId)
      parties[i].know_secret[t.secret_revealed] = true;
}

bool know_signature(Party p, Tx t, Key key) {
  int i;
  if(p.know_key[key]) return true;
  if(t.num >= TX_NUM) return false;
  for(i = 0; i < p.known_signatures_size; i++) {
    Signature s = p.known_signatures[i];
    if(s.tx_num == t.num and s.input_nonce == bc[t.input].nonce
             and s.key == key)
      return true;
  }
  return false;
}

bool can_create_input_script(Party p, Tx t) {
  OutputScript o = bc[t.input].out_script;
  if(o.standard) 
    return know_signature(p, t, o.key);
  if(o.script == 0) 
    return (know_signature(p, t, C_KEY) and p.know_secret[0] 
            and t.reveals_secret and t.secret_revealed == C_SEC)
        or (know_signature(p, t, C_KEY) and know_signature(p, t, R_KEY));
  return false;
}

bool can_send(Party p, Tx t) {
  return t.status == UNSENT and is_valid(t) and can_create_input_script(p, t);
}

void try_to_send(Party p, Tx& t) {
  if(can_send(p, t))
    send(t);
}

bool own(Party p, Tx t) {
  OutputScript out = t.out_script;
  return t.status == CONFIRMED and out.standard and p.know_key[out.key];
}

int count_owners(Tx t) {
  int res = 0;
  for(i : PartyId)
    if(own(parties[i], t))
      res++;
  return res;
}

int hold_bitcoins(Party p) {
  int res = 0;
  for(i : TxId)
    if(own(p, bc[i]) and count_owners(bc[i]) == 1)
      res += bc[i].value;
  return res;
}

bool sig_sent;
Signature sig;
const Key ADV_KEY = C_KEY;

const TxId INPUT = 0;
const TxId COMMIT = 1;
const TxId OPEN = 2;
const TxId FUSE = 3;

urgent chan send_sig;

Tx create_prot_tx(TxId num) {
  Tx res;
  if(num == INPUT)  { res = create_standard_tx(num, INPUT,  C_KEY); 
          res.value = 1; res.status = CONFIRMED; }
  if(num == COMMIT) { res = create_standard_tx(num, INPUT,  C_KEY); 
          res.out_script = create_nss(0); }
  if(num == OPEN)   { res = create_standard_tx(num, COMMIT, C_KEY); 
          res.reveals_secret = true; res.secret_revealed = C_SEC; }
  if(num == FUSE)   { res = create_standard_tx(num, COMMIT, R_KEY); 
          res.timelock = PROT_TIMELOCK; }
  return res;
}

void init_prot() {
  parties[ALICE].know_key[C_KEY] = true;
  parties[ALICE].know_secret[C_SEC] = true;
  parties[BOB].know_key[R_KEY] = true;
  parties[ADVERSARY] = parties[ALICE];
}

void init_bc() {
  int i;
  for(i : TxId) {
    if(i < PROT_TX_NUM)
      bc[i] = create_prot_tx(i);
    else
      bc[i] = create_standard_tx(i, i - PROT_TX_NUM, ADV_KEY);
    if(bc[i].timelock == 0)
      bc[i].timelock_passed = true;
  }
}

// SYSTEM DECLARATIONS

BlockChainAgentTA = BlockChainAgent();
HelperTA = Helper();
AliceTA = Alice(parties[ALICE]);
BobTA = Bob(parties[BOB]);
AdversaryTA = Adversary(parties[ADVERSARY]);

system AdversaryTA, BobTA, BlockChainAgentTA, HelperTA;
\end{Verbatim}
}
